Linear regression and its inference on noisy network-linked data

Linear regression on network-linked observations has been an essential tool in modeling the relationship between response and covariates with additional network structures. Previous methods either lack inference tools or rely on restrictive assumptions on social effects and usually assume that networks are observed without errors. This paper proposes a regression model with nonparametric network effects. The model does not assume that the relational data or network structure is exactly observed and can be provably robust to network perturbations. Asymptotic inference framework is established under a general requirement of the network observational errors, and the robustness of this method is studied in the specific setting when the errors come from random network models. We discover a phase-transition phenomenon of the inference validity concerning the network density when no prior knowledge of the network model is available while also showing a significant improvement achieved by knowing the network model. Simulation studies are conducted to verify these theoretical results and demonstrate the advantage of the proposed method over existing work in terms of accuracy and computational efficiency under different data-generating models. The method is then applied to middle school students' network data to study the effectiveness of educational workshops in reducing school conflicts.

==> Append-Example.tex <==

\section{Additional results of the simulation examples}\label{sec:additional-sim}

Table~\ref{tab:Controlled-SBM-Chisq} summarizes the type-I error probability of the $\chi^2$ test from the setting $\gamma = (0, 0, 0, 0)^T$ in the configuration of Section~\ref{sec:sim}. It shows the desired type-I error control to test $H_0: \alpha = 0$


\begin{table}[H]
\centering
\caption{The type-I error probability of the $\chi^2$ test for $\gamma$ when the network is generated from the SBM and $\gamma = 0$. }
\label{tab:Controlled-SBM-Chisq}
\begin{tabular}{l|rrrr}
  \hline
\multirow{2}{*}{Method} & \multirow{2}{*}{$n$} & \multicolumn{3}{c}{average expected degree} \\ 
%\hline
 &  & $2\log{n}$ & $\sqrt{n}$ & $n^{2/3}$  \\ 
   \hline
 \multirow{3}{*}{SP}& 1000& 0.0490 & 0.0497 & 0.0510 \\
 & 2000  & 0.0504 & 0.0497 & 0.0506 \\ 
 & 4000  & 0.0496 & 0.0490 & 0.0501 \\ 
\hline
 \multirow{3}{*}{SP-SBM} & 1000& 0.0496 & 0.0500 & 0.0511 \\ 
& 2000 & 0.0504 & 0.0495 & 0.0503 \\ 
 & 4000 & 0.0499 & 0.0493 & 0.0500 \\  
   \hline
\end{tabular}
\end{table}



As a counterpart of the study in Section~\ref{sec:sim}, we generate networks from the DCBM. For the DCBM, the degree parameters are generated from a uniform distribution between 0.2 and 1.  All of the other configurations remain the same, as in the previous setting. Table~\ref{tab:Controlled-DCBM-Ratio} shows the average bias-SD ratio for $\hat{\beta}_2, \hat{\beta}_3$ and $\hat{\beta}_3$ under the DCBM, while Table~\ref{tab:Controlled-DCBM-Coverage} shows the empirical coverage of the 95\% confidence intervals in this setting. The high-level message remains similar to the SBM setting and matches the theory. It can be seen that both versions of SP are valid for large enough $n$ when $\varphi_n = n^{2/3}$, while the parametric version also works for $\varphi_n = 2\sqrt{n}$. However, the advantage of the parametric version is smaller compared with the SBM setting because the DCBM estimation is more complicated.  Lastly, Table~\ref{tab:Controlled-DCBM-Chisq} shows the type I error probability of the $\chi^2$ test, in which the validity is evident.


\begin{table}[H]
\centering
\caption{The average theoretical bias-SD ratio for $\beta_2, \beta_3$ and $\beta_4$ when the network is generated from the DCBM.}
\label{tab:Controlled-DCBM-Ratio}
\begin{tabular}{l|rrrr}
  \hline
\multirow{2}{*}{Method} & \multirow{2}{*}{$n$} & \multicolumn{3}{c}{average expected degree} \\ 
%\hline
 &  & $2\log{n}$ & $\sqrt{n}$ & $n^{2/3}$  \\ 
  \hline
\multirow{3}{*}{SP}& 1000 & 1.509 & 0.675 & 0.268 \\ 
 & 2000 & 2.084 & 0.681 & 0.204 \\ 
 & 4000 & 3.105 & 0.636 & 0.167 \\  
\hline
\multirow{3}{*}{SP-DCBM} &1000 & 0.950 & 0.286 & 0.096 \\ 
 & 2000 & 1.040 & 0.238 & 0.089 \\ 
 & 4000 & 1.470 & 0.180 & 0.081 \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{The average coverage coverage probability of 95\% confidence intervals of $\beta_2, \beta_3, \beta_4$ when the network is generated from the DCBM.}
\label{tab:Controlled-DCBM-Coverage}
\begin{tabular}{l|rrrr}
  \hline
\multirow{2}{*}{Method} & \multirow{2}{*}{$n$} & \multicolumn{3}{c}{average expected degree} \\ 
%\hline
 &  & $2\log{n}$ & $\sqrt{n}$ & $n^{2/3}$  \\ 
  \hline
\multirow{3}{*}{SP}& 1000& 0.775 & 0.912 & 0.944 \\
 & 2000 & 0.605 & 0.901 & 0.946 \\ 
 & 4000  & 0.329 & 0.892 & 0.947 \\ 
\hline
\multirow{3}{*}{SP-DCBM} & 1000  & 0.881 & 0.943 & 0.950 \\ 
 & 2000 & 0.848 & 0.945 & 0.948 \\  
 & 4000 & 0.754 & 0.946 & 0.951 \\ 
   \hline
\end{tabular}
\end{table}




\begin{table}[H]
\centering
\caption{The type-I error probability of the $\chi^2$ test for $\gamma$ when the network is generated from the DCBM and $\gamma = 0$.}
\label{tab:Controlled-DCBM-Chisq}
\begin{tabular}{l|r|rrr}
  \hline
 \multirow{2}{*}{Method} & \multirow{2}{*}{$n$} & \multicolumn{3}{c}{average expected degree} \\ 
%\hline
 & & $2\log{n}$ & $\sqrt{n}$ & $n^{2/3}$  \\ 
   \hline
\multirow{3}{*}{SP}& 1000& 0.0518 & 0.0514 & 0.0506 \\ 
& 2000  & 0.0515 & 0.0517 & 0.0497 \\ 
 & 4000  & 0.0508 & 0.0504 & 0.0501 \\
 \hline
 \multirow{3}{*}{SP-DCBM} & 1000 & 0.0512 & 0.0515 & 0.0502 \\ 
 & 2000 & 0.0518 & 0.0510 & 0.0492 \\  
 & 4000 & 0.0498 & 0.0489 & 0.0498 \\  
   \hline
\end{tabular}
\end{table}



Table~\ref{tab:DCSBM-compare} shows the comparison of our methods with the benchmark methods in the DCBM setting.


\begin{table}[H]
\centering
\caption{The mean squared error (MSE) $\times 10^2$ of $\e Y$ when the network is generated from the DCBM with $n=1000, p=4, K=4$ with three types of individual effects.  } 
{\small
\label{tab:DCSBM-compare}
\begin{tabular}{l|l|rrrrrrr}
  \hline
 indiv. effects &   avg. degree & SP & SP-DCBM & OLS & SIM &RNC & SP-L & SP-DCBM-L\\ 
  \hline
\multirow{4}{*}{eigenspace} & $2\log{n}$ & 11.07 & 6.70 & 41.51 & 29.63 & 12.28 & 41.51 & 41.51 \\  
& $\sqrt{n}$ & 4.47 & 1.26 & 41.51 & 27.89 & 10.95 & 41.51 & 41.51 \\ 
 & $n^{2/3}$ & 1.23 & 0.38 & 41.51 & 24.22 & 9.47 & 41.51 & 41.51 \\ 
\hline
\multirow{4}{*}{$\gamma = 0$} & $2\log{n}$ & 0.14 & 0.14 & 0.12 & 27.48 & 0.26 & 0.13 & 0.12 \\ 
 & $\sqrt{n}$ & 0.14 & 0.13 & 0.12 & 26.00 & 0.64 & 0.13 & 0.13 \\  
 & $n^{2/3}$ & 0.13 & 0.13 & 0.12 & 25.34 & 1.57 & 0.13 & 0.12 \\ 
\hline
\multirow{4}{*}{smooth} & $2\log{n}$& 25.20 & 25.20 & 25.20 & 28.34 & 16.03 & 12.69 & 17.92 \\ 
  & $2\sqrt{n}$  & 23.83 & 23.83 & 23.81 & 25.24 & 14.79 & 12.00 & 12.26 \\ 
  & $n^{2/3}$ & 26.21 & 26.22 & 26.20 & 26.70 & 12.80 & 13.20 & 15.00 \\ 
   \hline
\end{tabular}
}
\end{table}



\newpage

\section{Adolescents’ social activity study}\label{sec:additional-data}


The AddHealth study \citep{harris2009national} is a longitudinal study about various health-related behaviors of students in grade 7--12 in the U.S..  In this section, we use a subset of the AddHealth data to study the gender and racial effects on social activity diversity.  The data set contains 82 local communities, and each local community contains one public high school. The students listed up to 10 friends and how many different types of social activities they had with each friend. The average number of social activities per friend is calculated as a measure of social activity diversity as an important factor in mental health \citep{sherbourne1988role,wildes2002life}. Besides this, the gender, grade, and race information are also available for each student. In some of the local communities, a feeder middle school of the high school is also included. In this case, the data set also contains the school labels of the students. We want to learn whether there are significant gender and racial differences in the social activity diversity level of the students. This type of analysis may bring insights about health-related behaviors in adolescents' life. In the context, it is evident that social network information should be incorporated in modeling because each social activity may involve multiple students, and ignoring this factor may lead to misleading results. 


The SP method is applied to all 82 data sets (local communities) and we always report the summary results with the 0.05 FDR control \citep{benjamini1995controlling}. Out of the 82 data sets,  72 data sets present significant gender effect, and 14 data sets reveal significant racial effect. The network effect is significant in 37 communities. Here, we pick the largest network with significant network effects in the data set ($n=2152$ nodes and two schools) to show a detailed analysis. The network is shown in Figure~\ref{fig:comm36}, in which the node sizes represent the estimated $\alpha$ in the SP. Large size indicates that the individual is believed to have higher social diversity. 




\begin{figure}[h]
\vspace{-1cm}
\centering
\includegraphics[trim = 20 20 20 40, clip, width=0.8\textwidth]{Comm36-withSchool.pdf}
\vspace{-1cm}
\caption{The friendship network of 2152 students with school information.}
\label{fig:comm36}
\end{figure}



Cross-validation of the network \citep{li2016network} indicates that neither of the block models is proper. Therefore, focus is instead placed on the model-free version of the SP on this data set.  The p-value for the $\chi^2$ test of $\gamma$ is close to 0, indicating a significant network effect. 
Multiple insignificantly different levels of the race variable are then merged, resulting in a binary variable of ``white" and ``non-white" (reference level), and the models are fit again. In both cases, $r$ is estimated to be zero indicating no strong confounding between the covariates and the network structure. And the estimate $\beta$ is the sole characterization of the covariate effects. Both two versions of model fitting results are shown in Table~\ref{tab:comm36-coef}. 




\begin{table}[H]
\centering
\caption{Regression coefficients $\hat{\beta}$ and the confidence intervals from the largest local community in the data set.}
\label{tab:comm36-coef}
\begin{tabular}{l|rr|rr|rr|rr|rr|}
  \hline
  &\multicolumn{4}{c}{original variables}& \multicolumn{4}{c}{merged variables}\\
  \hline
  &\multicolumn{2}{c}{SP}&\multicolumn{2}{c}{OLS}& \multicolumn{2}{c}{SP}&\multicolumn{2}{c}{OLS}\\
  \hline
 & coef. & p-val.  & coef. & p-val.  & coef. & p-val.  & coef. & p-val. \\ 
  \hline
  sex & 0.180 & $<10^{-9}$ &  0.173 & $<10^{-7}$ & 0.180 & $<10^{-8}$ & 0.172 & $<10^{-7}$\\ 
  grade & 0.246 & $<10^{-3}$ &  0.206 & $<10^{-5}$& 0.245 & $<10^{-7}$  & 0.203 & $<10^{-5}$ \\ 
  school & 0.003 & 0.476 & -0.039 & 0.380 & 0.006 & 0.448  & -0.035 & 0.427 \\ 
race: white & 0.484 & 0.075  & 0.746 & 0.030 & 0.380 & $<10^{-7}$ & 0.598 & $<10^{-9}$\\ 
race: black & 0.038 & 0.456  & 0.044 & 0.901 &--&--&--&--\\ 
race: hispanic  & 0.106 & 0.376  & 0.163 & 0.633 &--&--&--&--\\ 
race: other & 0.167 & 0.315  & 0.189 & 0.593 &--&--&--&--\\ 
 \hline
\end{tabular}
\end{table}


It can be seen that sex has a significant effect, indicating that girls tend to involve in 0.18 more social activities on average. The grade is also statistically significant, indicating increasingly diverse social activities among students as they grow up. In these refined results, The race effect estimated by OLS is about 1.5 times the effect size estimated by the SP. OLS also estimates an obviously weaker effect on grade.   These differences can be explained by network interference, demonstrated in Figure~\ref{fig:comm36-race}.   It appears that friendship ties between students exhibit evident race preference --- most white (non-white) students tend to make friends with other white (nonwhite) students. A similar pattern is also observed for the grade, as expected because students tend to make friends with others in the same grade. These correlations between the network structure and the variables explains why our model gives very different estimates of racial and grade effects. Notice that the proposed model includes the standard linear model as a special case, and the $\chi^2$ test indicates a strong social effect. We believe that the proposed model may be preferable as it is reasonable to believe that social effects exist in this situation and the inference framework can test the significance of the network effects. 
   



\begin{figure}
%\vspace{-1cm}
\centering
\includegraphics[trim = 20 60 20 50,clip,width=0.49\textwidth]{Comm36-withRace.pdf}
\includegraphics[trim = 20 60 20 50,clip,width=0.49\textwidth]{Comm36-withGrade.pdf}
\caption{The friendship network of 2152 students with race and grade information.}
\label{fig:comm36-race}
\end{figure}


==> Data.tex <==
\section{ School conflict reduction study}\label{sec:conflict}
In \cite{paluck2016changing}, an experiment is conducted to study the impacts of educational workshops on reducing conflicts in schools. The experimenters randomly selected 26 middle schools in New Jersey in which they held educational workshops. In each school, the experimenters first determined a group of eligible students. A small proportion of them was selected (randomly after gender and race blocking) to participate in bi-monthly educational workshops about how to help reduce school conflicts. Students were also asked to name who they “spend time with” in the survey, and the answers were used to construct the social network structure. We ignore the directions of edges and treat two students as connected as long as either one identifies the other as a connection. For each school, we take the largest connected component of the social network as the final data. In total, there are 9,429 students in our analysis. 


 
 
We follow a similar analysis as in  \cite{paluck2016changing}.  In particular, students provided how much their friends ``influence their way of dealing with conflicts", and how much their friends ``talked about how to change the school climate". These two variables are averaged as the response, as a measure of ``friends' support of reducing conflicts". The covariates include whether the student participates the workshops, the proportion of the student's friends involved in the workshops, and 
those selected based on the significance in an OLS model fitting, including gender, whether the student is Asian or not, and the number of conflicts the student experienced in the past year (summarized in nine categories of conflicts in the survey). The school effects are also included to accommodate the individual school differences. 

Applying the model-free version of our SP method,  the $\chi^2$ test results in a very small p-value ($<10^{-5}$), indicating that the social effect is significant. The estimated $r$ is zero, so there is no confounding between the covariates and the network, and $\xi$ is trivially zero. The covariate effects are given in Table~\ref{tab:Conflict-Inference}, in comparison with the OLS results without modeling the social effect. The school effects are not presented due to space limit. 

For the first three covariates, the estimated effects are similar between our method and the OLS estimates. The estimates reveal that female students and asian students tend to observe more supports from friends about reducing school conflicts. The more conflicts one experiences, the more supports they would see from friends. Meanwhile, the estimates of the educational program effects by OLS and  our method are very different. Neither of the two covariates about the educational program are estimated to be significant in OLS, while both of them have reasonably small p-values under our model. Because our method includes the OLS as a special case, and the $\chi^2$ test indicates a strong network effect,  we believe the inference of our method is more reasonable. Our conclusion can also be supported by the original analysis of experimenters \citep{paluck2016changing}, who delivered the same conclusion. However, the analysis of \cite{paluck2016changing} takes the experiment design and sampling probability into consideration with additional assumptions about the spill-over effects of the educational workshops and is based on complicated causal inference methods. Therefore, their conclusion is about the stronger causal relation. In contrast, our method does not take advantage of the design, nor do we know whether the network cohesion assumption has an explicit correspondence to the widely used spill-over effects assumptions. So our conclusion is not causal. We leave the development of causal inference under the current framework for future work. 

\begin{table}[h]
\centering
\caption{Regression coefficients of covariate effects in the school conflict example.}
\label{tab:Conflict-Inference}
\begin{tabular}{l|rr|rr|rr}
  \hline
  &\multicolumn{2}{c}{Our method}&\multicolumn{2}{c}{OLS}\\
  \hline
 & coef. & p-val.& coef. & p-val.  \\ 
  \hline
  Gender: Boy & -0.140 & $<10^{-5}$ & -0.146& $ <10^{-5}$ \\  
  Race: Asian & 0.175 & $<10^{-5}$ & 0.150& $ <10^{-5}$ \\  
  Conflicts in the past year & 0.034 & $<10^{-5}$ &0.038& $ <10^{-5}$ \\  
  Educated & 0.068 & 0.010  & 0.048 & 0.097 \\ 
  Proportion of educated friends & 0.239 & 0.029  & 0.046 & 0.71 \\  
   \hline
\end{tabular}
\end{table}

In addition to the current example, we also apply our method to analyze socially active levels of adolescents based on the AddHealth study of \cite{harris2009national}. The details are included in Appendix~\ref{sec:additional-data}.





==> Intro.tex <==
\section{Introduction}\label{sec:intro}

Nowadays, networks appear frequently in many areas, including social sciences, transportation, and biology. In most cases, networks are used to represent relationships or interactions between units of a complex (social, physical, or biological) system, so analyzing network data may render crucial insights into the dynamics and/or interaction mechanism of the system. One particular, yet commonly encountered, situation is when a group of units is observed connected by a network and a set of attributes for each of these units is available.  Such data sets are sometimes called network-linked data \citep{li2016prediction, li2019high} or multiview network data \citep{gao2019testing}. Network-linked data are widely available in almost all fields involving network analysis about social effects \citep{michell1996peer,pearson2003drifting}, collaborations \citep{ji2016coauthorship,su2019testing}, and causal experiments \citep{basse2018limitations,basse2018model}. In such a data set, rich information is available from the perspective of both the individual attributes and the network, and the challenge is to find proper statistical methods to incorporate both. Consider the situation where, for each node $i$ of the network, we observe $({x}_i, y_i)$, in which ${x}_i \in \bR^p$ is a vector of covariates while $y_i \in \bR$ is a scalar response. In particular, we aim for a regression model of $y_i$ against ${x}_i$ that also takes the network information into account. Such a model arises naturally in any problem when a prediction model or inference of a specific attribute is of interest. 


Although the systematic study of regression on network-linked data has only recently begun to attract interest in statistics \citep{li2016prediction,zhu2017network,su2019testing}, it has been studied in econometrics by many authors, who mostly focused on multiple networks \citep{manski1993identification,lee2007identification,bramoulle2009identification} or longitudinal data \citep{jackson2007relating, manresa2013estimating}.  Social effects are typically observed in the form that connected units share similar behaviors or properties. Such similarity or correlation may be due to either \emph{homophily}, where social connections are established because of similarity, or \emph{contagion}, where individuals become similar through the influence of their social ties. In general, one cannot distinguish homophily from contagion in a single snapshot of observational data \citep{shalizi2011homophily}, as in our setting. Therefore, the two directions of causality will not be distinguished,  and this type of generic similarity between connected nodes will be called ``network cohesion", as in \cite{li2016prediction, li2019high}. %Traditionally, investigations focused on three different types of social effects: endogenous effect, exogenous (or contextual) effect and external (or correlated) effect  \citep{manski1993identification}. Roughly speaking, the endogenous effect refers to the dependence of one's response on its neighbors' responses, while the exogenous effect refers to the dependence of one's response on its neighbors' covariates. The external effect measures the similarity or correlation introduced by other latent information (not included in covariates or responses). 
A significant class of models for such network regression problems is the class of autoregressive models, which is based on ideas in spatial statistics.   The spatial autoregressive models have been widely used in econometrics, such as in \cite{manski1993identification,lee2007identification,bramoulle2009identification,hsieh2016social,zhu2017network}, to name a few.  A common form for such a model is 
%\begin{equation}\label{eq:SIM}
$$y_i = \gamma \Big(\frac{1}{n_i}\sum_{i'\sim i}y_{i'}\Big) + X\beta + \frac{1}{n_i}\Big(\sum_{i'\sim i}x_{i'}\Big)^T\eta + \epsilon,$$
%\end{equation}
where $y_i$ is the response, $x_i$ is the covariate vector and $n_i$ is the number of neighbors of $i$ (the notation $i\sim i'$ indicates that $i$ and $i'$ are connected). In this model, the neighborhood averages of the response  and covariates are  used to model the social effect. The parameters $\gamma$ and $\eta$ are typically called ``endogenous" and ``exogenous" effects, respectively, while $\beta$ is the standard regression slope. This class of models is also called the ``linear in means" model or social interaction model (SIM).  When multiple networks for different populations are available, the intercept can be treated as a group effect, called  the``external effect" \citep{manski1993identification,lee2007identification,lee2010specification}.  The SIM framework, though it has been a popular setup for regression on network-linked data,  suffers from two crucial drawbacks. The first comes from its restrictive parametric form of the social effect. Assuming social effect in the form of autoregressive neighborhood average (or summation)  is far from realistic, and such a stringent assumption significantly limits the usefulness of the framework. As shown in \cite{li2016prediction} and also in our empirical study, the restrictive assumption of social effect leads to poor prediction performance. The second limitation  comes from the  assumption that the network structure is precisely observed from the data. In practice, it is well known that most network data are subject to errors, due to missingness \citep{lakhina2003sampling,butts2003network,
clauset2005accuracy}, observational errors \citep{handcock2010modeling,
rolland2014proteome,le2017estimating,
khabbazian2017novel,newman2018estimating,
lunagomez2018evaluating}, or data collection method \citep{wu2018link, rohe2019critical}. If the imprecise network is used in SIM, the model is ill-defined and the inference would also be problematic, as shown by \cite{chandrasekhar2011econometrics}.



In this paper, a new regression model to fit the network-linked data is proposed that addresses both drawbacks mentioned above. The new model is based on a flexible network effect assumption and is robust to network observational errors. It also allows us to perform tests and construct confidence intervals for the model parameters. 
Our theoretical analysis provides the support for model estimation and inference and quantifies the magnitude of network observational errors under which the inference remains robust. Moreover, in the random network perturbation scenario, the tradeoff between the available information of the network structure and the level of robustness of the statistical inference is characterized. In its most difficult setting, when no prior knowledge about the network model is available, the result reveals a phase-transition phenomenon at the network average degree of $\sqrt{n}$, above which the inference is asymptotically correct, and below which the inference becomes invalid. The inference  could remain valid for much sparser networks if more information about the network structure is available. For example, when the network model is known and an effective parametric estimation can be applied, the sparsity requirement can be relaxed to $\log{n}$.  To the best of  our knowledge, this paper is the first work that addresses the inference of the network-linked regression models and accounts for the network observational errors.


Related to the network-linked model proposed in this paper is the semi-parametric model called ``regression with network cohesion" (RNC), introduced by \cite{li2016prediction}. In their model, the network effect is represented by individual parameters that are assumed to be ``smooth" over the network, and a similar idea is used in a few other statistical estimation settings \citep{wang2014trend,zhao2016significance,fan2018approximate}.  Despite its flexibility of social effect assumption and excellent  predictive performance, the RNC model lacks a valid inference framework and cannot be applied in many modern applications where statistical inference is needed \citep{ogburn2018challenges, su2019testing}. The result of \cite{li2019high} indicates that the RNC estimator fails to guarantee valid inference under reasonable assumptions unless additional assumptions such sparsity are made \citep{zhao2016significance}. Moreover, little is known about the robustness of the RNC method to network observational errors, although preliminary results have been obtained in a particular scenario of network sparsification \citep{sadhanala2016graph,li2016prediction}. In contrast, our model does not assume the smoothness of network effects as in the RNC method. Instead, we use a general relational subspace to define the social effects. As can be seen later, the proposed model overcomes both of the two aforementioned limitations of RNC and is computationally more efficient.

Table~\ref{tab:model-compare} gives a high-level comparison between the proposed model and two popular benchmark regression models (discussed previously) in three aspects: the flexibility of modeling social effects, the availability of an inference method, and the provable robustness to the network perturbation. The model we introduced in this paper is the only one of the three which renders all of the  desired properties.
\begin{table}[H]
\caption{Comparison between the proposed method and two other popular methods for network-linked data.}\label{tab:model-compare}
\begin{center}
\begin{tabular}{|c|c|c|c|}  
    \cline{1-4}
    \multicolumn{1}{|c|}{Models} & social effect flexibility & inference & network robustness  \\
    \hline
    SIM \citep{manski1993identification} & \xmark & \cmark & \xmark \\
    \hline
    RNC \citep{li2016prediction} & \cmark & \xmark & \xmark \\
    \hline
    Current method & \cmark & \cmark & \cmark \\
    \hline
\end{tabular}
\end{center}
\end{table}


The rest of the paper is organized as follows. Section~\ref{sec:model} introduces our model and the corresponding statistical inference algorithm. Section~\ref{secsec:generic-inference} and Section~\ref{sec:theory} are devoted to our main theoretical results; the generic theory for model estimation consistency and the asymptotic inference is given in Section~\ref{secsec:generic-inference}; then, under the random network modeling framework, detailed discussions of the technical requirement are introduced in  Section~\ref{sec:theory}. Extensive simulation experiments are given in Section~\ref{sec:sim} to verify our theory and compare our method with a few benchmark methods mentioned above. Section~\ref{sec:conflict} demonstrates the usefulness of the proposed method in analyzing the gender and racial effects on social activities among adolescents. Concluding remarks and future directions are discussed in Section~\ref{sec:conclusion}. The proofs of all theoretical results and additional real data analysis are given in the supplementary material.





==> bounding_delta2_initial_version.tex <==
\subsubsection{Bounding $\delta_2$}

Since $\tilde{R} = RW$ and $\tilde{U} = UV$, it follows that
$$
\tilde{R}_{\cdot i} \tilde{U}^T_{\cdot i} = RW_{\cdot i} (UV_{\cdot i})^T = RW_{\cdot i} V_{\cdot i}^T U^T.
$$
Similarly, since $R^T\hat{U} = \hat{W}\hat{\Sigma}\hat{V}^T$, $\hat{R} = R\hat{W}$ and $\breve{U} = \hat{U}\hat{V}$,
$$
\hat{R}_{\cdot i} \breve{U}^T_{\cdot i} = R\hat{W}_{\cdot i} (\hat{U}\hat{V}_{\cdot i})^T = R\hat{W}_{\cdot i} \hat{V}_{\cdot i}^T \hat{U}^T.
$$
Therefore
\begin{eqnarray*}
\delta_2 &=& R W_{\cdot(r+1):(r+s)}\Gamma(1-\Gamma^2)^{-1} V_{\cdot(r+1):(r+s)}^TU^T - R \hat{W}_{\cdot(r+1):(r+s)}\hat{\Gamma}(1-\hat{\Gamma}^2)^{-1} \hat{V}_{\cdot(r+1):(r+s)}^T\hat{U}^T
\end{eqnarray*}
By Davis-Kahan lemma, there exists a rotation matrix $O\in\mathbb{R}^{K\times K}$ such that 
$$
\|\hat{U}O-U\| \le \xi.
$$
Using $\hat{U}^T = O(\hat{U}O)^T$, we have
$$
\|\hat{U}^T - OU^T\|\le \xi.
$$
Let $\delta_2'$ be the expression obtained from $\delta_2$ by replacing $\hat{U}^T$ with $OU^T$. Then by David-Kahan lemma,
$$
\|\delta_2'-\delta_2\| \le \xi\cdot \|(1-\hat{\Gamma}^2)^{-1}\| = \frac{\xi}{1-\|\hat{\Gamma}\|^2} \le \frac{\xi}{1-(\sigma_{r+1}+\xi)^2}.
$$
Since $\|R\|=\|U\| = 1$, 
$$
\|\delta_2'\| \le \left\|W_{\cdot(r+1):(r+s)}\Gamma(1-\Gamma^2)^{-1} V_{\cdot(r+1):(r+s)}^T - \hat{W}_{\cdot(r+1):(r+s)}\hat{\Gamma}(1-\hat{\Gamma}^2)^{-1} \hat{V}_{\cdot(r+1):(r+s)}^TO\right\|.
$$
Recall that $R^TU = W\Sigma V^T$, $R^T\hat{U}O=\hat{U}\hat{\Sigma}\hat{V}^TO$ and $\|R^TU-R^T\hat{U}O\|\le \xi$. By the bound \eqref{eq: singular decomposition restriction bound} of Lemma~\ref{lem: projection bound}, if
$$
\min\{1-\sigma_{r+1},\sigma_{r+s}\}-4\xi >0
$$
then
\begin{eqnarray*}
\left\|W_{\cdot(r+1):(r+s)}\Gamma V_{\cdot(r+1):(r+s)}^T - \hat{W}_{\cdot(r+1):(r+s)}\hat{\Gamma} \hat{V}_{\cdot(r+1):(r+s)}^TO\right\| \le \frac{3\xi}{\min\{1-\sigma_{r+1},\sigma_{r+s}\}-4\xi}.
\end{eqnarray*}
Therefore by Lemma~\ref{lem: unorthogonal projection bound}, if 
$$
\sigma_{r+1} + \frac{6\xi}{\min\{1-\sigma_{r+1},\sigma_{r+s}\}-4\xi} < 1
$$
then 
\begin{eqnarray*}
\|\delta_2\| &\le& \|\delta_2'\| + \|\delta_2'-\delta_2\| \\
&\le& 
\frac{3\cdot\frac{3\xi}{\min\{1-\sigma_{r+1},\sigma_{r+s}\}-4\xi}}{\left(1-\sigma_{r+1}^2 -2\cdot\frac{3\xi}{\min\{1-\sigma_{r+1},\sigma_{r+s}\}-4\xi}\right)^2} + \frac{\xi}{1-(\sigma_{r+1}+\xi)^2}\\
&=& O(\xi),
\end{eqnarray*}
where $\xi$ is the upper bound in David-Kahan lemma such that $\|\hat{U}O-U\| \le \xi$ for some rotation matrix $O$.

\begin{lem}[Bound on singular vectors and partial singular decomposition]\label{lem: projection bound}
Let $X, \hat{X}$ be $p\times k$ matrices with singular decompositions
$$
X = U\Sigma V^T, \quad \hat{X} = \hat{U}\hat{\Sigma}\hat{V}^T.
$$
Let $\eta$ be a set of singular values of $X$, $\eta^c$ be the set of remaining singular values of $X$ and 
$\Delta = \min_{\sigma\in\eta,\sigma'\in\eta^c}|\sigma-\sigma'|.$
Denote by $U_\eta$ the matrix whose columns are left singular vectors of $X$ with corresponding singular values in $\eta$; define $V_{\eta}, \hat{U}_\eta$ and $\hat{V}_\eta$ similarly.   
Assume that $\|X\|\le 1$, $\|\hat{X}\|\le 1$ and $\Delta>4\|\hat{X}-X\|$. Then
\begin{eqnarray}
\label{eq: projection difference bound}
\max\left\{\|\hat{U}_\eta\hat{U}_\eta^T-U_\eta U_\eta^T\|,\|\hat{V}_\eta\hat{V}_\eta^T-V_\eta V_\eta^T\|\right\}  &\le& \frac{2\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}, \\
\label{eq: singular decomposition restriction bound}
\Big\|\sum_{i\in \eta} \sigma_i U_{\cdot i} V_{\cdot i}^T - \sum_{i\in \eta} \hat{\sigma}_i \hat{U}_{\cdot i} \hat{V}_{\cdot i}^T\Big\| &\le& \frac{3\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}. 
\end{eqnarray} 
\end{lem}
\begin{proof}
Note that $X^TX$ and $\hat{X}^T\hat{X}$ are symmetric matrices with eigenvectors $V_{\cdot i}$, $\hat{V}_{\cdot i}$ and eigenvalues being squares of singular values of $X$ and $\hat{X}$, respectively. Also, by the triangle inequality, 
\begin{eqnarray*}
\|\hat{X}^T\hat{X}-X^TX\| = \|(\hat{X}-X)^T\hat{X}-X^T(\hat{X}-X)\| \le 2\|\hat{X}-X\|. 
\end{eqnarray*}
Therefore by Theorem 7.3.1 of \cite{Bhatia1996},
\begin{eqnarray*}
\|\hat{V}_\eta\hat{V}_\eta^T-V_\eta V_\eta^T\| &\le& \frac{\|\hat{X}^T\hat{X}-X^TX\|}{\Delta - 2\|\hat{X}^T\hat{X}-X^TX\|} \le \frac{2\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}.
\end{eqnarray*}
A similar bound holds for $\|\hat{U}_\eta\hat{U}_\eta^T-U_\eta U_\eta^T\|$ if we consider $XX^T$ instead of $X^TX$, and \eqref{eq: projection difference bound} is proved. 

It remains to show \eqref{eq: singular decomposition restriction bound}. Let $S$ and $\hat{S}$ be diagonal matrices with $\sigma_i,i\in \eta$ and $\hat{\sigma}_i,i\in \eta$ on the diagonal, respectively. For every unit vector $x$, we need to bound 
$\|U\eta S V_\eta^Tx - \hat{U}\eta \hat{S} \hat{V}_\eta^Tx\|$. Let $H=V_\eta V_\eta^T, H^\perp = I - H$, $\hat{H} = \hat{V}_\eta\hat{V}_\eta^T$ and $\hat{H}^\perp = I - \hat{H}$. Since
$$
x = Hx + H^\perp x = \hat{H}x+\hat{H}^\perp x,
$$
it follows that
$$
U\eta S V_\eta^Tx - \hat{U}\eta \hat{S} \hat{V}_\eta^Tx = U\eta S V_\eta^T H x - \hat{U}\eta \hat{S} \hat{V}_\eta^T \hat{H}x = XHx - \hat{X}\hat{H}x.
$$
By \eqref{eq: projection difference bound}, we have
\begin{eqnarray*}
\|\hat{X} \hat{H}x - \hat{X} Hx\| \le \|(\hat{H}-H)x\| \le \frac{2\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}.
\end{eqnarray*}
Therefore
\begin{eqnarray*}
\|U\eta S V_\eta^Tx - \hat{U}\eta \hat{S} \hat{V}_\eta^Tx\| &\le& \|XHx - \hat{X}Hx\| + \|\hat{X} Hx-\hat{X} \hat{H}x\|\\
&\le& \|X - \hat{X}\| + \frac{2\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}\\
&\le& \frac{3\|\hat{X}-X\|}{\Delta-4\|\hat{X}-X\|}.
\end{eqnarray*} 
Since $x$ is an arbitrary unit vector, \eqref{eq: projection difference bound} is proved.
\end{proof}

\begin{lem}[Unorthogonal projection bound]\label{lem: unorthogonal projection bound}
Let $X, \hat{X}$ be two matrices of the same size with singular decompositions
$$
X = U\Sigma V^T, \quad \hat{X} = \hat{U}\hat{\Sigma}\hat{V}^T.
$$
Assume that $\|X\|<1$, $\|\hat{X}\|<1$ and $\|X\|^2 +2\|\hat{X}-X\|<1$. Then
\begin{eqnarray*}
\left\|U\Sigma(1-\Sigma^2)^{-1} V^T - \hat{U}\hat{\Sigma}(1-\hat{\Sigma}^2)^{-1} \hat{V}^T\right\| &\le& \frac{3\|X-\hat{X}\|}{(1-\|X\|^2 -2\|\hat{X}-X\|)^2}.
\end{eqnarray*}
\end{lem}

\begin{proof}
Since $\|\Sigma\|=\|X\|<1$ and $\|\hat{\Sigma}\|=\|\hat{X}\|<1$, we have
$$
\Sigma(1-\Sigma^2)^{-1} = \sum_{i=0}^\infty \Sigma^{2i+1},\qquad \hat{\Sigma}(1-\hat{\Sigma}^2)^{-1} = \sum_{i=0}^\infty \hat{\Sigma}^{2i+1}.  
$$
Therefore series 
\begin{eqnarray*}
U\Sigma(1-\Sigma^2)^{-1} V^T - \hat{U}\hat{\Sigma}(1-\hat{\Sigma}^2)^{-1} \hat{V}^T &=&
\sum_{i=0}^\infty \left(U\Sigma^{2i+1}V^T-\hat{U}\hat{\Sigma}^{2i+1}\hat{V}^T\right)\\
&=& \sum_{i=0}^\infty \left(U\Sigma V^T V \Sigma^{2i}V^T-\hat{U}\hat{\Sigma}\hat{V}^T\hat{V}\hat{\Sigma}^{2i}\hat{V}^T\right)\\
&=& \sum_{i=0}^\infty \left(X V \Sigma^{2i}V^T-\hat{X}\hat{V}\hat{\Sigma}^{2i}\hat{V}^T\right)\\
&=& \sum_{i=0}^\infty \left(X Y^{2i}-\hat{X}\hat{Y}^{2i}\right),
\end{eqnarray*}
where 
$Y = V\Sigma V^T$ and $\hat{Y} = \hat{V}\hat{\Sigma}\hat{V}^T$. Since $X^TX = Y^2$ and $\hat{X}^T\hat{X}=\hat{Y}^2$, it follows that $\|Y^2\|<1$ and
\begin{eqnarray*}
\|\hat{Y}^2 -Y^2\|\le\|\hat{X}^T(\hat{X}-X)\|+\|(\hat{X}-X)X\| \le 2\|\hat{X}-X\|.
\end{eqnarray*}
By the triangle inequality and the assumption of the lemma,
$$
\|\hat{Y}^2\|\le\|Y^2\|+ 2\|\hat{X}-X\| = \|X\|^2+ 2\|\hat{X}-X\| <1.
$$
Therefore $\sum_{i=0}^\infty Y^{2i}$ and $\sum_{i=0}^\infty \hat{Y}^{2i}$ are convergent series. By the triangle inequality, we have
\begin{eqnarray*}
\Big\|\sum_{i=0}^\infty \left(X Y^{2i}-\hat{X}\hat{Y}^{2i}\right)\Big\| &=&\Big\| \sum_{i=0}^n (X-\hat{X})Y^{2i} + \sum_{i=0}^\infty \hat{X}(Y^{2i}-\hat{Y}^{2i}) \Big\| \\
&\le& \|X-\hat{X}\|\cdot \Big\|\sum_{i=0}^\infty Y^{2i}\Big\| + \Big\|\sum_{i=0}^\infty Y^{2i}-\sum_{i=0}^\infty \hat{Y}^{2i}\Big\|\\
&=& \|X-\hat{X}\|\cdot\|(1-Y^2)^{-1}\| + \Big\|(1-\hat{Y}^2)^{-1}-(1-Y^2)^{-1}\Big\|\\
&=& \|X-\hat{X}\|\cdot\|(1-Y^2)^{-1}\|+\Big\|(1-\hat{Y}^2)^{-1}(\hat{Y}^2-Y^2)(1-Y^2)^{-1}\Big\|\\
&\le& \|X-\hat{X}\|\cdot\|(1-Y^2)^{-1}\|+\|\hat{Y}^2-Y^2\|\cdot \|(1-\hat{Y}^2)^{-1}\|\cdot\|(1-Y^2)^{-1}\|\\
&\le& \|X-\hat{X}\|\cdot\|(1-Y^2)^{-1}\|+2\|\hat{X}-X\|\cdot \|(1-\hat{Y}^2)^{-1}\|\cdot\|(1-Y^2)^{-1}\|.
\end{eqnarray*}
Note that $\|(1-Y^2)^{-1}\| = (1-\|Y^2\|)^{-1}=(1-\|X\|^2)^{-1}$ and
$$
\|(1-\hat{Y}^2)^{-1}\| = \frac{1}{1-\|\hat{Y}^2\|}\le \frac{1}{1-\|Y^2\| -2\|\hat{X}-X\|} = \frac{1}{1-\|X\|^2 -2\|\hat{X}-X\|}.
$$
Putting these inequalities together, we get
\begin{eqnarray*}
\Big\|\sum_{i=0}^\infty \left(X Y^{2i}-\hat{X}\hat{Y}^{2i}\right)\Big\| &\le& \frac{3\|X-\hat{X}\|}{(1-\|X\|^2 -2\|\hat{X}-X\|)^2}
\end{eqnarray*}
and the proof is complete.
\end{proof}

